Scalar actions in Lean's mathlib

Scalar actions are ubiquitous in mathematics, and therefore it is valuable to be able to write them succinctly when formalizing. In this paper we explore how Lean 3's typeclasses are used by mathlib for scalar actions with examples, illustrate some of the problems which come up when using them such as compatibility of actions and non-definitionally-equal diamonds, and note how these problems can be solved. We outline where more work is needed in mathlib in this area.

==> main-dot2tex-fig1.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (has_scalar) at (100.0bp,22.5bp) [draw,draw=none] {\scriptsize\lean{has_scalar}};
  \node (mul_action) at (71.0bp,43.5bp) [draw,draw=none] {\scriptsize\lean{mul_action}};
  \node (smul_with_zero) at (129.0bp,43.5bp) [draw,draw=none] {\scriptsize\lean{smul_with_zero}};
  \node (mul_action_with_zero) at (129.0bp,64.5bp) [draw,draw=none] {\scriptsize\lean{mul_action_with_zero}};
  \node (distrib_mul_action) at (50.0bp,64.5bp) [draw,draw=none] {\scriptsize\lean{distrib_mul_action}};
  \node (module) at (123.0bp,85.5bp) [draw,draw=none] {\scriptsize\lean{module}};
  \node (algebra) at (123.0bp,106.5bp) [draw,draw=none] {\scriptsize\lean{algebra}};
  \node (mul_semiring_action) at (55.0bp,85.5bp) [draw,draw=none] {\scriptsize\lean{mul_semiring_action}};
  \node (has_mul) at (244.0bp,22.5bp) [draw,draw=none] {\scriptsize\lean{has_mul}};
  \node (mul_zero_class) at (219.0bp,43.5bp) [draw,draw=none] {\scriptsize\lean{mul_zero_class}};
  \node (monoid) at (270.0bp,43.5bp) [draw,draw=none] {\scriptsize\lean{monoid}};
  \node (monoid_with_zero) at (238.0bp,64.5bp) [draw,draw=none] {\scriptsize\lean{monoid_with_zero}};
  \node (semiring) at (238.0bp,85.5bp) [draw,draw=none] {\scriptsize\lean{semiring}};
  \node (comm_semiring) at (238.0bp,106.5bp) [draw,draw=none] {\scriptsize\lean{comm_semiring}};
  \draw [->] (mul_action) ..controls (80.597bp,36.213bp) and (81.7bp,35.49bp)  .. (has_scalar);
  \draw [->] (smul_with_zero) ..controls (119.4bp,36.213bp) and (118.3bp,35.49bp)  .. (has_scalar);
  \draw [->] (mul_action_with_zero) ..controls (107.47bp,56.446bp) and (102.57bp,54.842bp)  .. (mul_action);
  \draw [->] (mul_action_with_zero) ..controls (129.0bp,57.749bp) and (129.0bp,57.594bp)  .. (smul_with_zero);
  \draw [->] (distrib_mul_action) ..controls (56.526bp,57.596bp) and (56.872bp,57.283bp)  .. (mul_action);
  \draw [->] (module) ..controls (124.54bp,79.623bp) and (124.57bp,79.54bp)  .. (mul_action_with_zero);
  \draw [->] (module) ..controls (99.169bp,78.297bp) and (89.804bp,75.86bp)  .. (distrib_mul_action);
  \draw [->] (algebra) ..controls (123.0bp,99.815bp) and (123.0bp,99.726bp)  .. (module);
  \draw [->] (mul_semiring_action) ..controls (53.487bp,78.749bp) and (53.446bp,78.594bp)  .. (distrib_mul_action);
  \draw [->] (mul_zero_class) ..controls (227.07bp,36.366bp) and (227.8bp,35.809bp)  .. (has_mul);
  \draw [->] (monoid) ..controls (262.58bp,37.077bp) and (261.36bp,36.186bp)  .. (has_mul);
  \draw [->] (monoid_with_zero) ..controls (232.25bp,57.749bp) and (232.09bp,57.594bp)  .. (mul_zero_class);
  \draw [->] (monoid_with_zero) ..controls (249.35bp,56.764bp) and (251.42bp,55.535bp)  .. (monoid);
  \draw [->] (semiring) ..controls (238.0bp,78.749bp) and (238.0bp,78.594bp)  .. (monoid_with_zero);
  \draw [->] (comm_semiring) ..controls (238.0bp,99.749bp) and (238.0bp,99.594bp)  .. (semiring);
  \draw [gray,->] (has_mul) ..controls (195.17bp,22.5bp) and (163.55bp,22.5bp)  .. (has_scalar);
  \draw [gray,->] (mul_zero_class) ..controls (183.16bp,43.5bp) and (175.52bp,43.5bp)  .. (smul_with_zero);
  \draw [gray,->] (monoid) ..controls (255.78bp,51.116bp) and (251.05bp,53.031bp)  .. (246.5bp,54.0bp) .. controls (230.63bp,57.383bp) and (116.49bp,56.76bp)  .. (100.5bp,54.0bp) .. controls (99.027bp,53.746bp) and (97.53bp,53.425bp)  .. (mul_action);
  \draw [gray,->] (monoid_with_zero) ..controls (195.78bp,64.5bp) and (186.68bp,64.5bp)  .. (mul_action_with_zero);
  \draw [gray,->] (semiring) ..controls (196.32bp,85.5bp) and (172.79bp,85.5bp)  .. (module);
  \draw [gray,->] (comm_semiring) ..controls (187.36bp,106.5bp) and (168.38bp,106.5bp)  .. (algebra);
%
\end{tikzpicture}


==> main-dot2tex-fig2.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\node (addiAB) at (53.0bp,29.0bp) [draw,draw=none] {\scriptsize\lean{add_comm_monoid (ι → A →+ B)}};
  \node (moduleiAB) at (150.0bp,7.0bp) [draw,draw=none] {\scriptsize\lean{module ℕ (ι → A →+ B)}};
  \node (addAB) at (70.0bp,51.0bp) [draw,draw=none] {\scriptsize\lean{add_comm_monoid (A →+ B)}};
  \node (moduleAB) at (150.0bp,29.0bp) [draw,draw=none] {\scriptsize\lean{module ℕ (A →+ B)}};
  \node (addB) at (70.0bp,72.5bp) [draw,draw=none] {\scriptsize\lean{add_comm_monoid B}};
  \node (moduleB) at (150.0bp,51.0bp) [draw,draw=none] {\scriptsize\lean{module ℕ B}};
  \draw [blue,->] (addiAB) ..controls (91.037bp,20.157bp) and (101.02bp,18.098bp)  .. (moduleiAB);
  \draw [blue,->] (addAB) ..controls (64.495bp,43.523bp) and (64.367bp,43.373bp)  .. (addiAB);
  \draw [green,->] (addAB) ..controls (100.9bp,42.275bp) and (108.56bp,40.36bp)  .. (moduleAB);
  \draw [green,->] (addB) ..controls (67.914bp,65.603bp) and (67.9bp,65.45bp)  .. (addAB);
  \draw [blue,->] (addB) ..controls (72.782bp,65.603bp) and (72.8bp,65.45bp)  .. (addAB);
  \draw [red,->] (addB) ..controls (101.67bp,63.781bp) and (112.05bp,61.249bp)  .. (moduleB);
  \draw [red,->] (moduleAB) ..controls (147.88bp,21.523bp) and (147.87bp,21.373bp)  .. (moduleiAB);
  \draw [green,->] (moduleAB) ..controls (152.83bp,21.523bp) and (152.84bp,21.373bp)  .. (moduleiAB);
  \draw [red,->] (moduleB) ..controls (150.0bp,45.275bp) and (150.0bp,45.187bp)  .. (moduleAB);
%
\end{tikzpicture}

